Pollution and Mortality: Evidence from early 20th Century Sweden

Economic growth in Sweden during the early 20th Century was largely driven by industry. A significant contributor to this growth was the installation of different kinds of engines used to power factories. We use newly digitized data on engines and their energy source by industry sector, and combine this with municipality-level data of workers per industry sector to construct a new variable reflecting economic output using dirty engines. In turn, we assess the average externality of dirty output on mortality in the short-run, as defined by deaths over the population in the baseline year. Our results show substantial increases of up to 17% higher mortality in cities where large increases to dirty engine installations occurred, which is largely driven by the elderly. We also run a placebo test using clean powered industry and find no effect on mortality.

==> DD_new/First_stages.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump to 2nd decile}&\multicolumn{1}{c}{Jump to 3rd decile}&\multicolumn{1}{c}{Jump to 4th decile}&\multicolumn{1}{c}{Jump to 5th decile}&\multicolumn{1}{c}{Jump to 6th decile}&\multicolumn{1}{c}{Jump to 7th decile}&\multicolumn{1}{c}{Jump to 8th decile}&\multicolumn{1}{c}{Jump to 9th decile}\\
\midrule
ATT                 &     62.1558\sym{***}&     63.5080\sym{**} &    113.7046\sym{***}&    132.9960\sym{***}&    246.6973\sym{***}&    274.1827\sym{***}&    231.3039\sym{***}&    469.7577\sym{***}\\
                    &   (17.9862)         &   (26.7766)         &   (29.3684)         &   (31.7296)         &   (47.1678)         &   (41.3975)         &   (49.9558)         &  (114.8532)         \\
\midrule
Adj. R-squared      &                     &                     &                     &                     &                     &                     &                     &                     \\
Obs.                &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/First_stages_log.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      1.0958\sym{***}&      0.3049         &      0.2173         &      0.1554         &      0.2480\sym{***}&      0.1505\sym{*}  &      0.1359\sym{*}  &      0.1633\sym{**} \\
                    &    (0.3259)         &    (0.1981)         &    (0.1495)         &    (0.1028)         &    (0.0950)         &    (0.0865)         &    (0.0820)         &    (0.0757)         \\
\midrule
Adj. R-squared      &                     &                     &                     &                     &                     &                     &                     &                     \\
Obs.                &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_14_to_29ATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      0.2350         &      0.2704         &     -0.5242         &      0.0267         &      0.1943         &      0.5384\sym{***}&      0.0200         &      0.1131         \\
                    &    (0.4215)         &    (0.2921)         &    (0.3442)         &    (0.2125)         &    (0.3214)         &    (0.1954)         &    (0.1872)         &    (0.2059)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_1_to_13ATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      0.0218         &     -0.1090         &     -0.1091         &      0.2610         &      0.1711         &     -0.0775         &     -0.2633\sym{*}  &     -0.2839\sym{*}  \\
                    &    (0.3173)         &    (0.2541)         &    (0.2329)         &    (0.2272)         &    (0.2238)         &    (0.1256)         &    (0.1375)         &    (0.1719)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_30_to_49ATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      0.0364         &     -0.0616         &     -0.3255         &      0.4405\sym{**} &      0.2920         &      0.0900         &      0.0013         &     -0.0869         \\
                    &    (0.3800)         &    (0.2343)         &    (0.3237)         &    (0.2045)         &    (0.2357)         &    (0.1742)         &    (0.1684)         &    (0.1748)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_50_to_74ATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      0.1985         &     -1.5113\sym{**} &      0.5435         &      0.8156\sym{*}  &     -0.3593         &      0.2732         &      0.1902         &      0.0182         \\
                    &    (0.5450)         &    (0.6734)         &    (0.5997)         &    (0.4711)         &    (0.3466)         &    (0.2438)         &    (0.2044)         &    (0.2989)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_75_and_overATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      0.8849\sym{**} &     -0.0201         &      0.1757         &     -0.0231         &      0.0741         &      0.1012         &      0.2005         &     -0.5098\sym{**} \\
                    &    (0.4251)         &    (0.6274)         &    (0.3834)         &    (0.2705)         &    (0.3182)         &    (0.2561)         &    (0.1895)         &    (0.2592)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_all_agesATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      1.4781         &     -1.4388         &     -0.0141         &      1.4103\sym{*}  &      0.7200         &      1.0093         &      0.0417         &     -0.9445         \\
                    &    (1.0032)         &    (1.2747)         &    (0.9601)         &    (0.7932)         &    (0.6834)         &    (0.6475)         &    (0.4272)         &    (0.6580)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}


==> DD_new/Mortality_under_1ATT.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{longtable}{l*{8}{c}}
\toprule\endfirsthead\midrule\endhead\midrule\endfoot\endlastfoot
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{Jump 2nd dec.}&\multicolumn{1}{c}{Jump 3rd dec.}&\multicolumn{1}{c}{Jump 4th dec.}&\multicolumn{1}{c}{Jump 5th dec.}&\multicolumn{1}{c}{Jump 6th dec.}&\multicolumn{1}{c}{Jump 7th dec.}&\multicolumn{1}{c}{Jump 8th dec.}&\multicolumn{1}{c}{Jump 9th dec.}\\
\midrule
ATT                 &      0.1016         &     -0.0071         &      0.2256         &     -0.1104         &      0.3478\sym{*}  &      0.0841         &     -0.1069         &     -0.1951\sym{*}  \\
                    &    (0.2998)         &    (0.3519)         &    (0.1692)         &    (0.1720)         &    (0.1994)         &    (0.1568)         &    (0.1086)         &    (0.1167)         \\
\midrule
N                   &                     &                     &                     &                     &                     &                     &                     &                     \\
\bottomrule
\multicolumn{9}{l}{\footnotesize Clustered standard errors in parentheses.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<.1\), \sym{**} \(p<.05\), \sym{***} \(p<.01\)}\\
\end{longtable}
}

